RemixTape: Enriching Narratives about Metrics with Semantic Alignment and Contextual Recommendation

The temporal dynamics of quantitative metrics or key performance indicators (KPIs) are central to conversations in enterprise organizations. Recently, major business intelligence providers have introduced new infrastructure for defining, sharing, and monitoring metric values. However, these values are often presented in isolation and appropriate context is seldom externalized. In this design study, we present REMIXTAPE, an application for constructing structured narratives around metrics. With design imperatives grounded in prior work and a formative interview study, REMIXTAPE provides a hierarchical canvas for collecting and coordinating sequences of line chart representations of metrics, along with the ability to externalize situational context around them. REMIXTAPE includes affordances to semantically align and annotate juxtaposed charts and text, as well as recommendations of complementary charts based on metrics already present on the canvas. We evaluated REMIXTAPE in a study in which six enterprise data professionals reproduced and extended partial narratives. They appreciated REMIXTAPE as a novel alternative to dashboards, galleries, and slide presentations for supporting conversations about metrics. We conclude with a reflection on our design choices and process, with a call to define a conceptual foundation for remixing in the context of visualization.

==> listings/reco-algo.tex <==
\SetAlFnt{\small\tt}
\begin{algorithm}[t!]
    recommendations = []\\
    currentScene = getScene(selectedCard, canvas)\\
    leftCard = getLeftChartCard(selectedCard, currentScene)\\
    rightCard = getRightChartCard(selectedCard, currentScene)\\
    \uIf{isEmpty(selectedCard)}{
        \uIf{isEmpty(currentScene)}{
            metricRecos = getSceneStartMetricRecos(selectedCard, canvas)\\
            recommendations.push(metricRecos)
        }
        \uElseIf{isNotEmpty(leftCard)}{
            \uIf{hasFilter(leftCard)}{
                overviewReco = getOverviewCard(leftCard, currentScene)\\
                recommendations.push(overviewReco)
            }
            \vspace{.5em}
            filterRecos = getFilterRecos(leftCard, currentScene)\\
            recommendations.push(filterRecos)\\
            
            \vspace{.5em}
            metricRecos = getMetricSwitchRecos(selectedCard, canvas, rightCard)\\
            recommendations.push(metricRecos)
        }
        \uElseIf{isNotEmpty(rightCard)}{
            \uIf{hasFilter(rightCard)}{
                overviewReco = getOverviewCard(rightCard, currentScene)\\
                recommendations.push(overviewReco)
            }
            \vspace{.5em}
            metricRecos = getMetricSwitchRecos(selectedCard, canvas, rightCard)\\
            recommendations.push(metricRecos)
        }
    }
	\textbf{return} recommendations
    \caption{\small{\texttt{getRecommendations(selectedCard, canvas)}}}
    \label{algo:recommendation}
\end{algorithm}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/03-x-scenario.tex <==
%------------------------------------------------------------
\subsection{Usage Scenario}
\label{sec:remixing:scenario}
%------------------------------------------------------------

We now describe a usage scenario to motivate \remixtape's design and illustrate how the tool helps \revision[author]{people prepare and deliver} interactive presentations.

Imagine Sarah, a real estate analyst for the King County region in Washington, USA, is using \remixtape~to create a presentation about COVID-19 and its impact on the local housing market.
She has access to two datasets: one containing metrics about COVID-19 and the other containing metrics about home sales.
% , both for the King County region.
The COVID-19 dataset contains metrics such as \metric{Positives}, \metric{Hospitalizations}, and \metric{Deaths} reported at a \emph{daily} frequency spanning from February 2020 to April 2022.
The housing dataset contains metrics including \metric{Homes Sold}, \metric{Days on Market}, and \metric{Median Sale Price} but is reported at a \emph{monthly} frequency from January 2018 to April 2022 \textbf{(D1)}.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/scenario-combined-wide-hires.pdf}
    \caption{Using \remixtape~to \revision[author]{prepare} a presentation about COVID-19 and housing sales. Sub-figure captions summarize the system states.}
    \label{fig:scenario}
\end{figure*}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/scenario-2.pdf}
    \caption{Examples of \vizcard~actions. (A) Clicking the horizontal region above a chart provides options to filter, split, or fade out specific time periods. (B) Clicking the vertical region to the right of a chart adds a horizontal reference line to emphasize specific values along the y-axis.}
    \label{fig:scenario-2}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/present-mode.pdf}
    \caption{\remixtape's presentation mode. Scenes and cards are enlarged and all editing operations are disabled. Annotations (horizontal markers or faded out portions of a chart) and interactive links between text and charts are preserved to facilitate dynamic narration.}
    \label{fig:present-mode}
\end{figure}

\vspace{.25em}
\noindent\textbf{Starting with suggested metrics.}
Sarah starts her presentation by adding a scene and a visualization card (`\vizcard') to the canvas.
To help Sarah choose a metric to start her presentation, \remixtape~scans through the underlying data and suggests line charts depicting five metrics across the two datasets that might be interesting to consider based on their variability over time (Figure~\ref{fig:scenario}A).
Intrigued by the spike in the number of \metric{Positives} for COVID-19, Sarah adds it to the \vizcard.

\vspace{.25em}
\noindent\textbf{Filtering metrics and adding interactive notes.}
Noticing that \metric{Positives} does not have values prior to Feb 2020, Sarah filters the chart to only show data since Feb 2020 (Figure~\ref{fig:scenario-2}A).
Sarah detects two prominent spikes in the data, one towards end of 2021 and another towards the end 2020.
She makes a note of these spikes in a \textcard~and links {\small{\faMagic}} her notes to the \vizcard~(Figure~\ref{fig:scenario}B) to interactively highlight the relevant portions of the chart (\textbf{D4}).
% Within the \textcard, Sarah mentions the time periods of the two spikes (Nov 2021-Feb 2022, Nov 2020-Feb 2021) in her notes and links~{\small{\faMagic}} these notes to the \vizcard.

\vspace{.25em}
\noindent\textbf{Comparing metrics through juxtaposition.}
Next, to compare the two spikes Sarah creates two clones~{\small{\faCopy}} of the \vizcard~showing \metric{Positives} and filters them to time periods corresponding to the two spikes (Nov 2021-Feb 2022, Nov 2020-Feb 2021).
Noticing that the y-axes are misaligned, Sarah synchronizes the cards align their y-axis scales (Figure~\ref{fig:scenario}C).
Using the juxtaposed and synchronized cards, Sarah notes that the recent peak is almost 9x that for the preceding year and also that the spike in 2021-2022 was around New Year's whereas the 2020-2021, the spike was around the Thanksgiving holiday in the US.

\vspace{.25em}
\noindent\textbf{Merging metrics and adding annotations.}
To explore other metrics that may be relevant for comparing the two peaks, Sarah copies the \vizcard~showing the peak for \metric{Positives} in Nov 2021-Feb 2022 and examines the system recommendations.
\remixtape~scans the underlying datasets to suggest metrics that exhibit a comparable trend to \metric{Positives} during that time (\textbf{D3}).
Seeing \metric{People Tested} in the recommendations, Sarah adds it to her scene as it can help contextualize the values for \metric{Positives} (Figure~\ref{fig:scenario}D).
As she adds the \metric{People Tested} metric to her scene, \remixtape~detects that the \vizcard{s} for the two metrics are juxtaposed, share a common time period on the x-axis, and have a comparable y-axis domain.
Based on these overlaps, the system provides an option to merge \raisebox{-.5em}{\includegraphics[height=1.5em]{figures/icons/merge.png}} the two cards into a multi-series line chart.
Sarah merges the two cards and similarly creates another card with a multi-series line chart of \metric{Positives} and \metric{People Tested} for the preceding year's spike (Nov 2020-Feb 2021).
Comparing the two multi-series line charts, Sarah notes that the rate of positives was also significantly higher for the recent spike ($\sim$36\% compared to $\sim$8\% the preceding year).
To emphasize this drastic difference in the number of \metric{Positives}, she also adds horizontal markers on the y-axes (Figure~\ref{fig:scenario-2}B) (\textbf{D4}).

\vspace{.25em}
\noindent\textbf{Manually specifying metrics.}
Having identified two time periods of interest for the COVID-19 metrics, Sarah expands her presentation to include metrics from the housing sales dataset.
Sarah starts a new scene and manually selects the \metric{Homes Sold} and \metric{Positives} metrics in the input panel.
To focus on the recent COVID spike noted in the first scene, she explicitly specifies Nov 2021-Feb 2022 as her time period of interest in the input panel.
\remixtape, in response, presents a multi-series line chart that combines the two metrics, implicitly aggregating the \metric{Positives} to match the monthly granularity of the \metric{Homes Sold} metric (Figure~\ref{fig:scenario}E).
Sarah adds this chart to the scene and similarly creates a second \vizcard~spanning Nov 2020-Feb 2021.

\vspace{.25em}
\noindent\textbf{Switching to an overview.}
Looking at the two \vizcard{s}, Sarah notices a dip in \metric{Homes Sold} around Nov-Dec, coinciding with the spike in \metric{Positives} for both years.
% Curious about how she can build upon this observation in her presentation, she adds a new \vizcard~and requests system recommendations.
As she adds a new card to build upon this observation, \remixtape~detects that the current scene only contains two filtered cards and in turn, suggests an overview card spanning the entire data time range of Jan 2018-Apr 2022 (Figure~\ref{fig:scenario}F) (\textbf{D3}).
Inspecting the overview card recommendation Sarah realizes that the drops in \metric{Homes Sold} during Nov-Dec were a common occurrence even before the pandemic.
She updates the scene to include a \vizcard~showing the values for the months before Feb 2020 and makes a note of this observation.

\vspace{.25em}
\noindent\textbf{Finding related metrics.}
Finally, to see metrics that relate to home sales, Sarah adds a new \vizcard~showing only the \metric{Home Sales} metric and peruses through the system recommendations.
Comparing the available metrics to \metric{Home Sales}, \remixtape~suggests \metric{New Listings} as the most related metric (Figure~\ref{fig:teaser}) (\textbf{D3}).
Visually sifting through the comparable trends, Sarah creates a merged \vizcard~composing of \metric{Home Sales} and \metric{New Listings} (similar to Figure~\ref{fig:scenario}D).
\newline

\noindent{}With two scenes covering four metrics across two datasets and different time periods, as well as a set of \textcard{s} containing her observations about those metrics, Sarah switches to the ``Present Mode" (Figure~\ref{fig:present-mode}) to look through her canvas from a viewer's perspective.
Sarah then shares the canvas with her colleagues to further discuss how the trend of housing sales is following its natural progression despite the COVID-19 data patterns.

==> sections/acknowledgements.tex <==
%% if specified like this the section will be committed in review mode
The authors conducted this research while at Tableau. The authors thank Zach Morrissey, Marlen Promann, Carolyn Tweedy, and our study participants.


==> sections/archive/scenario-Aug31.tex <==
%------------------------------------------------------------
\subsection{Usage Scenario}
\label{sec:remixing:scenario}
%------------------------------------------------------------

We now describe a usage scenario to motivate \remixtape's design and illustrate how the tool helps author interactive presentations.

Imagine Sarah, a real estate analyst for the King County region in Washington, USA, is using \remixtape~to create a presentation about COVID-19 and its impact on the local housing market.
She has access to two datasets: one containing metrics about COVID-19 and the other containing metrics about house sales, both for the King County region.
The COVID-19 dataset contains six metrics (e.g., \metric{Positives}, \metric{Hospitalizations}, \metric{Deaths}) reported at a \emph{daily} frequency spanning from February 2020 to April 2022.
The housing dataset also contains six metrics (e.g., \metric{Homes Sold}, \metric{Days on Market}, \metric{Median Sale Price}) but is reported at a \emph{monthly} frequency from January 2018 to April 2022.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/scenario-combined-wide.pdf}
    \caption{Using \remixtape~to author a presentation about COVID-19 and housing sales. Sub-figure captions summarize the system states. \todo{Make E larger}}
    \label{fig:scenario}
\end{figure*}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/scenario-2.pdf}
    \caption{Examples of \vizcard~actions. (A) Clicking the horizontal region above a chart provides options to filter, split, or fade out specific time periods. (B) Clicking the vertical region to the right of a chart adds a horizontal reference line to emphasize specific values along the y-axis.}
    \label{fig:scenario-2}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/present-mode.pdf}
    \caption{\remixtape's presentation mode. Scenes and cards are enlarged and all editing operations are disabled. Annotations (horizontal markers or faded out portions of a chart) and interactive links between text and charts are preserved to facilitate dynamic narration. \todo{show interactivity}}
    \label{fig:present-mode}
\end{figure}

\vspace{.25em}
\noindent\textbf{Starting with suggested metrics.}
Sarah starts her presentation by adding a scene and a visualization card (`\vizcard') to the canvas.
% Not having seen this data before, Sarah is unsure about which metrics to start with and clicks the ``Get Recommendations'' button.
% In response, \remixtape~scans through the underlying data and lists five metrics across the two datasets that might be interesting to consider based on their variability over time (Figure~\ref{fig:scenario}A).
To help Sarah choose a metric to start her presentation, \remixtape~scans through the underlying data and lists five metrics across the two datasets that might be interesting to consider based on their variability over time (Figure~\ref{fig:scenario}A).
Intrigued by the spike in the number of \metric{Positives} for COVID-19, Sarah chooses it from the list of recommendations as her first \vizcard.

\vspace{.25em}
\noindent\textbf{Filtering and adding interactive notes.}
Noticing that the metric does not have any values prior to February 2020, Sarah filters the chart to just show data since Feb 2020 (Figure~\ref{fig:scenaro-2}A).
Looking at the filtered chart, Sarah detects two prominent spikes in the data, one towards end of 2021 and another towards the end 2020.
To make a note of these observations, she creates a \textcard~alongside the \vizcard, adds notes about the two spikes, and links~{\small{\faMagic}} her notes to the \vizcard~showing \metric{Positives} (Figure~\ref{fig:scenario}B).
% Within the \textcard, Sarah mentions the time periods of the two spikes (Nov 2021-Feb 2022, Nov 2020-Feb 2021) in her notes and links~{\small{\faMagic}} these notes to the \vizcard.

\vspace{.25em}
\noindent\textbf{Comparing \vizcard{s} through juxtaposition.}
Having identified two time periods of interest, Sarah moves on to compare them.
To preserve the initial \vizcard~as context, Sarah creates two clones~{\small{\faCopy}} and filters them to time periods corresponding to the two spikes (Nov 2021-Feb 2022, Nov 2020-Feb 2021).
Looking at the juxtaposed cards (Figure~\ref{fig:scenario}C), she notices that the more recent peak was in the first week of January (around New Year's) whereas in 2020, the peak was in the last week of November (around the Thanksgiving holiday in the US).
Realizing that the y-axis scales are misaligned, Sarah clicks the y-axis of the right card and selects the ``Synchronize y domain" option to align the y-axis scales (Figure~\ref{fig:scenario}C).
The juxtaposed+aligned scales allow for easier comparison of the magnitude of the peaks, and Sarah notes that the recent peak is almost 9x that for the year before.

\vspace{.25em}
\noindent\textbf{Merging metrics.}
To explore other metrics that may be relevant for comparing the two peaks, Sarah clones the \vizcard~showing the peak for Nov 2021-Feb 2022, wondering which metric(s) to introduce in subsequent cards.
\remixtape~scans the data to suggest a list of metrics that exhibit a comparable trend to \metric{Positives} during the same time period of Nov 2021-Feb 2022.
Seeing \metric{People Tested} in the suggestions, Sarah adds it to her scene as it can help contextualize the values for the \metric{Positives} metric (Figure~\ref{fig:scenario}D).
As she adds the \metric{People Tested} to her scene, \remixtape~detects that the \vizcard{s} for the \metric{Positives} and \metric{People Tested} are juxtaposed, share a common time period on the x-axis, and have a comparable y-axis domain.
Based on these overlaps, the system provides an option to merge \todo{[MERGE\_ICON]} the two cards into a multi-series line chart.
Sarah merges the two cards and similarly creates a second card with a multi-series line chart of \metric{Positives} and \metric{People Tested} for the spike in the preceding year (Nov 2020-Feb 2021).
She compares the two multi-series line charts and adds notes to indicate that the rate of positives was significantly higher for the recent spike ($\sim$36\% compared to $\sim$7\% the preceding year).
To emphasize the drastic difference in the number of \metric{Positives}, Sarah also adds horizontal markers on the y-axes (Figure~\ref{fig:scenario-2}B).

\vspace{.25em}
\noindent\textbf{Manually specifying \vizcard{s}.}
% After creating the merged card, Sarah goes on to create a similar merged card for the spike in the preceding year.
% Specifically, she clones the \vizcard~showing the \metric{Positives} for Nov 2020-Feb 2021 and adds an empty \vizcard~after that.
% However, since she already knows the metric she wants to use, instead of asking for recommendations, Sarah directly clicks on the \metric{People Tested} metric in the left panel to get a \vizcard~showing its values over time.
% Sarah adds this to her scene and merges the two cards to get a new \vizcard~showing the \metric{Positives} and \metric{People Tested} metrics for Nov 2020-Feb 2021.
Having identified two time periods of interest for the COVID-19 metrics, Sarah expands her presentation to include metrics from the housing sales dataset and discuss the potential impact of the COVID-19 on the housing market.
Sarah starts a new scene and manually selects the \metric{Homes Sold} and \metric{Positives} metrics in the input panel.
Aware of the time period of the recent COVID spike from her first scene, she also specifies Nov 2021-Feb 2022 as her time period of interest in the input panel.
\remixtape, in response, returns line charts displaying the selected metrics, including a multi-series line chart that combines the two cross-dataset metrics, implicitly aggregating the \metric{Positives} to a monthly granularity (Figure~\ref{fig:scenario}E).
Sarah adds this chart to her scene and similarly creates a second \vizcard~spanning Nov 2020-Feb 2021.

\vspace{.25em}
\noindent\textbf{Switching back to an overview and finding related metrics.}
Looking at the two multi-series line charts, Sarah notices a dip in \metric{Homes Sold} around the November-December months, coinciding with the spike in \metric{Positives} for both years.
Curious about how she can build upon this observation in her presentation, she adds a new \vizcard~and requests system recommendations.
Detecting that she has only included two filtered cards in the current scene, \remixtape~suggests an overview card that spans the entire data time range of Jan 2018-Apr 2022 (Figure~\ref{fig:scenario}F).
Inspecting the overview card recommendation Sarah notices that the drops in \metric{Homes Sold} during November-December were a common occurrence even before the pandemic.
Correspondingly, she updates the scene to include a filtered \vizcard~showing the values for the months before Feb 2020 and makes a note of this observation.
Finally, to see metrics that relate to home sales, Sarah adds a new \vizcard~showing the \metric{Home Sales} metric and peruses through the system recommendations.
Comparing the available metrics to \metric{Home Sales}, \remixtape~suggests \metric{New Listings} as the most related metric (Figure~\ref{fig:teaser}).
Visually confirming the trends, Sarah creates a merged \vizcard~composing of \metric{Home Sales} and \metric{New Listings} (similar to Figure~\ref{fig:scenario}D).
\newline

\noindent{}With two scenes covering four metrics across two datasets and different time periods, as well as a set of \textcard{s} containing her observations about those metrics, Sarah switches to the ``Present Mode" (Figure~\ref{fig:present-mode}) to look through her canvas from a viewer's perspective.
Sarah then shares the canvas with her colleagues to further discuss how the trend of housing sales is following its natural progression and that number of COVID-19 related cases may not have directly impacted the real estate market.

==> sections/xx-limitations-and-future-work.tex <==
%============================================================
\section{Limitations and Future Work}
\label{sec:conclusion}
%============================================================

% \begin{itemize}
%     \item More viz types and customization features
%     \item Generalizing other data types
%     \item Recommendations for sequencing existing content in a scene/canvas
%     \item \cref{fig:remixtape-mobile}
%     \item Layout configuration options for presentation mode (e.g., one at a time, smaller or hidden text cards as notes)
%     \item Evaluation (\cite{ren2018reflecting,satyanarayan2019critical})
% \end{itemize}

The feedback from the preliminary user study helped us identify some immediate areas for improvement in \remixtape's interface as well as open research directions for future work.

\vspace{.5em}
\noindent\textbf{Supporting additional chart types and customization.}
\remixtape~currently only supports single- and multi-series line charts.
While these were sufficient to convey the underlying idea and gather user feedback, adding support for alternative representations including bar charts, or dual-axis charts combining both bars and lines, among others would be required to make the tool practically viable.
Besides additional chart types, another common topic that came up as an area for improvement was advanced support for formatting and customization (e.g., changing line colors, choosing font styles and sizes, configuring the layout of text and chart cards in presentation mode).

\vspace{.5em}
\noindent\textbf{Exploring sequence recommendations and \textcard~content suggestions.}
The current set of recommendations in \remixtape~help authors incrementally create a presentation by surfacing new metrics or charts that continue the narrative around an existing metric.
An alternative category of recommendations that came up during the study were recommendations for organizing/sequencing the content within a scene.
Specifically, participants wanted the ability to add a series of cards to a scene and then get ideas for how to order the cards to form potentially coherent narratives.
Along these lines, an opportunity for future work is to investigate how ideas from prior work on narrative sequencing~\cite{hullman2013deeper,lan2021understanding} and perception-based sequential visualization recommendations~\cite{kim2017graphscape,lin2020dziban} can be applied to suggest potentially interesting narrative sequences combining both charts and text.
Another category of recommendations that came up during multiple sessions were \textcard~content recommendations.
In particular, participants wanted the ability to link a \textcard~to a \vizcard~and get recommendations for potential points to highlight in the presentation.
Such recommendations are in line with the growing suite of natural language generation and ``auto-insight'' features in visualization tools~\cite{wang2019datashot,srinivasan2018augmenting,cui2019datasite}, and present compelling research opportunities to explore the integration of text and charts in the context of data-driven presentations.

\vspace{.5em}
\noindent\textbf{Conducting a more detailed evaluation.}
As with other visualization authoring tools, choosing an evaluation strategy for \remixtape~was a challenge requiring us to consider trade-offs between different criteria such as learnability, usability, workflow integration, and expressiveness~\cite{Amini2018DDS,satyanarayan2019critical}.
Following strategies from prior systems~\cite{ren2018reflecting}, we informed \remixtape's current version through a formative study and then evaluated it using a combination of replication and free-form authoring tasks.
These strategies collectively allowed us to get preliminary feedback on the tool's usability and learnability, and also the tool's creativity support to some extent.
However, more thoroughly evaluating the tool and understanding its expressiveness and creativity support calls for a longer term study that spans beyond a single 60-90 minute session.
To this end, an area for future work is to incorporate the system feedback from the current preliminary study and conduct longitudinal studies with authors using \remixtape~to create presentations involving metrics relevant to their job roles.
% “If I was not being timed on this, I would go down a rabbit hole” - would experiment with different ways to view case counts and days on market (P5)


\figRemixTapeMobile
